Full-Spectrum Out-of-Distribution Detection

Existing out-of-distribution (OOD) detection literature clearly defines semantic shift as a sign of OOD but does not have a consensus over covariate shift. Samples experiencing covariate shift but not semantic shift are either excluded from the test set or treated as OOD, which contradicts the primary goal in machine learning -- being able to generalize beyond the training distribution. In this paper, we take into account both shift types and introduce full-spectrum OOD (FS-OOD) detection, a more realistic problem setting that considers both detecting semantic shift and being tolerant to covariate shift; and designs three benchmarks. These new benchmarks have a more fine-grained categorization of distributions (i.e., training ID, covariate-shifted ID, near-OOD, and far-OOD) for the purpose of more comprehensively evaluating the pros and cons of algorithms. To address the FS-OOD detection problem, we propose SEM, a simple feature-based semantics score function. SEM is mainly composed of two probability measures: one is based on high-level features containing both semantic and non-semantic information, while the other is based on low-level feature statistics only capturing non-semantic image styles. With a simple combination, the non-semantic part is cancelled out, which leaves only semantic information in SEM that can better handle FS-OOD detection. Extensive experiments on the three new benchmarks show that SEM significantly outperforms current state-of-the-art methods. Our code and benchmarks are released in https://github.com/Jingkang50/OpenOOD.

==> sections/3_problem_statement.tex <==
\section{FS-OOD Problem Definition}
In this section, we formally define the proposed multi-source out-of-distribution (FS-OOD) detection problem. Let $\mathcal{X}$ and $\mathcal{Y}$ be the input and the label space, respectively, a data distribution is defined as a joint distribution $P(X, Y)$ over $\mathcal{X} \times \mathcal{Y}$. This joint distribution $P(X, Y)$ can be further decomposed into $P(X, Y) = P(Y|X) P(X) = P(X|Y) P(Y)$. It is generally assumed that the conditional distribution $P(Y|X)$ or $P(X|Y)$ remains relatively stable, while distribution shift occurs in either the marginal $P(X)$ or $P(Y)$, or both.

This work focuses on image classification tasks. Assume we have trained a classifier $f: \mathcal{X} \to \mathcal{Y}$ from a source dataset $\mathcal{S} = \{(\bm{x}, y)\}$ with $\bm{x}$ and $y$ denoting image and label respectively and $(\bm{x}, y) \sim P(X, Y)$. This classifier is deployed in a target dataset $\mathcal{T} = \{\bm{x}\}$ to predict the class label for each test image. In an OOD detection problem, we aim to identify whether a test image is drawn from the same data distribution as the source images, and allow the model to reject samples that are beyond the source distribution, so the decision-making process can be transferred to humans for better handling.

Different from existing research that assumes the source distribution $P(X, Y)$ is homogeneous, this work introduces a more challenging yet realistic setting called FS-OOD detection where the source distribution is \emph{heterogeneous}---the source images are drawn from a mixture of distributions rather than a single one. Formally, we have a collection of source distributions $\{ P^{(k)}(X, Y) \}_{k=1}^K$ where $K>1$ denotes the number of sources, and $P^{(k)}(X, Y) \neq P^{(k')}(X, Y)$ for $k, k' \in \{1, ..., K\}$ but $k \neq k'$. We assume all sources share the same label space so $P^{(k)}(Y) = P^{(k')}(Y)$, hence distribution shift occurs in $P(X)$. In practice, we might not be able to observe $K$.
